Online Learning with Off-Policy Feedback

We study the problem of online learning in adversarial bandit problems under a partial observability model called off-policy feedback. In this sequential decision making problem, the learner cannot directly observe its rewards, but instead sees the ones obtained by another unknown policy run in parallel (behavior policy). Instead of a standard exploration-exploitation dilemma, the learner has to face another challenge in this setting: due to limited observations outside of their control, the learner may not be able to estimate the value of each policy equally well. To address this issue, we propose a set of algorithms that guarantee regret bounds that scale with a natural notion of mismatch between any comparator policy and the behavior policy, achieving improved performance against comparators that are well-covered by the observations. We also provide an extension to the setting of adversarial linear contextual bandits, and verify the theoretical guarantees via a set of experiments. Our key algorithmic idea is adapting the notion of pessimistic reward estimators that has been recently popular in the context of off-policy reinforcement learning.

==> 9-unknown_pi.tex <==
\subsection{Prod with unknown behavior policy}
In the previous section we assumed to have access to the behavior policy $\pi_b$.
In this section, we present an alternative algorithm () which makes no such
assumption and still provides a meaningful regret bound.

The algorithm uses an estimated behavior policy $\hat{\pi}_t$, defined
using the information available up to and including time step $t$:
\begin{equation}\label{eq:pihat}
    \hat{\pi}_t(a) \doteq \frac{1}{t} \sum_{k=1}^{t} \One{A^b_k = a}.
\end{equation}
This estimator is then substituted to $\pi_b$ in the definition of the estimated
reward functions $\hat{r}_t$, which thus becomes
\begin{equation}
    \hat{r}_{t}(a) \doteq \frac{R^b_t \One{A^{b}_t = a }}{\hat{\pi}_t(a)} = 
    \frac{r_t(a) \One{A^{b}_t = a }}{\hat{\pi}_t(a)}.
\end{equation}

\begin{algorithm}
\caption{Prod with unknown behavior policy}\label{alg:prod2}
 \begin{algorithmic}
 \Procedure{PROD}{learning rate $\eta$}
     \State $w_1(a) \gets 1$
     \For{$t\gets 1,\dots,n$}
         \State $\pi_t(a) \gets w_t(a)/ \sum_{a\in\A} w_t(a)$
         \State play $A_t$ according to $\pi_t(\cdot)$
         \State observe $A^b_t$ and $R^b_t$
 
        \State $\hat{\pi}_{t}(a) \gets \frac{1}{t} \sum_{k=1}^t \One{ A^b_k = a}$
         \State $\hat{r}_{t}(a) \gets R^b_t \One{A^{b}_t = a }/ \hat{\pi}_t(a)$
 
         \State $w_{t+1}(a) \gets w_{t}(a)(1+\eta\cdot\hat{r}_{t}(a))$
 
     \EndFor
 \EndProcedure
 \end{algorithmic}
\end{algorithm}


\begin{theorem}\label{bound1}
By setting the learning rate $\eta$ to $\sqrt{\frac{\log K}{n}}$,
given any time-invariant compatator policy $\pi^*$, the regret incurred by
\cref{alg:prod2} can be bounded as:
$$
\E{\Reg(\pi^*)} \leq \dots
$$
\end{theorem}

To prove this bound, we start by showing that under a certain \textit{good event},
occurring with high probability and denoted as $E_t$ in the rest of the paper,
our estimate of the behavior policy $\hat{\pi}_t$ is close to the true value $\pi_b$.
Then, similarly to the previous section, we relate the estimated Regret
$\hat{\Reg}$ with the true Regret $\Reg$. This enables us to use once again
Prod's original Regret bound (\cref{eq:prod-bound}), which we then refine further.

% The full proof, which is given in the Appendix, relies on the following three lemmas.

\begin{lemma}
    Let $\delta_t\in(0,1)$. Then, for all actions $a\in\A$
    it holds with probability at least $1-\delta_t$ that:
    $$
    \abs{\hat{\pi}_t(a) - \pi_b(a) } < \sqrt{\frac{1}{2t} \log{\frac{2K}{\delta_t}}}
    $$
\begin{proof}
        Let $\epsilon_t\in\R_+$ and $\delta_t \doteq 2K\exp(-2t\epsilon^2_t)$.
        Define the event $\bar{E}_{ta}\doteq \abs{ \hat{\pi}_t(a) - \pi_b(a) } \geq \epsilon_t$
        and its negation $E_{ta} = \abs{ \hat{\pi}_t(a) - \pi_b(a) } < \epsilon_t$.
        Hoeffding's inequality gives us that $\P{\bar{E}_{ta}}\leq \delta_t/K$.
        Let $\bar{E}_t \doteq \cup_{a\in\A} \bar{E}_{ta}$. Then, its negation
        is $E_t = \cap_{a\in\A} E_{ta}$.
        Take an union bound over the actions, to get
        $\P{\bar{E}_t} \leq \suma \P{\bar{E}_{ta}} \leq \delta_t$
        Finally, we get $\P{E_t}\geq 1-\delta_t$.
    \end{proof}

\end{lemma}

We now show that in expectation $\hat{\Reg}$ is an upper-bound on the true regret
$\Reg$, by bounding each individual term.

\begin{lemma}
    Let $\delta_t\in(0,1)$ and $\epsilon_t \doteq \sqrt{\frac{1}{2t} \log{\frac{2K}{\delta_t}}}$. Then
    
    $$
    \E{\ip{\pi_t}{\hat{r}_t}} \leq \E{\ip{\pi_t}{r_t}} + \E*{\epsilon_t\frac{\pi_t(a)}{\hat{\pi}_t(a)} \given E_t} + 
t\delta_t
    $$

    \begin{proof}
        We start by conditioning on the good event $E_t$:
        \begin{align*}
                \E{\ip{\pi_t}{\hat{r}_t} \given E_t} &=  \E*{\suma \pi_t(a)\frac{r_t(a)\One{A^b_t=a}}{\hat{\pi}_t(a)} 
\given E_t} \\
            &= \E*{
                \E[\bigg]{\suma \pi_t(a)\frac{r_t(a)}{\hat{\pi}_t(a)} \given A^b_t=a}\P{A^b_t=a}
                + \E[\big]{\dots \given A^b_t \neq a}\P{A^b_t\neq a}
                \given E_t } \\
            &= \E*{\suma \pi_t(a)\frac{r_t(a)\pi_b(a)}{\hat{\pi}_t(a)} \given E_t} \\
            &\leq \E*{\suma \pi_t(a)\frac{r_t(a)(\hat{\pi}_t(a)+\epsilon_t)}{\hat{\pi}_t(a)} \given E_t} \\
            &= \E{\ip{\pi_t}{r_t}} + \E*{\epsilon_t\frac{\pi_t(a)}{\hat{\pi}_t(a)} \given E_t}
        \end{align*}
        Then we use the Law of total expectation to prove the desired bound
        \begin{align*}
            \E{\ip{\pi_t}{\hat{r}_t}} &= \E{\ip{\pi_t}{\hat{r}_t}\mid E_t}\P{E_t} + \E{\ip{\pi_t}{\hat{r}_t}\mid 
\bar{E}_t}\P{\bar{E}_t} \\
            &\leq \E{\ip{\pi_t}{r_t}} + \E*{\epsilon_t\frac{\pi_t(a)}{\hat{\pi}_t(a)} \given E_t} + t\delta_t
        \end{align*}
    \end{proof}
\end{lemma}


\begin{lemma}
    Let $\delta_t\in(0,1)$. For any action $a\in\A$ we have:
    $$
    r_t(a) \leq  \E{\hat{r}_t(a)} + \delta_t.
    $$

    \begin{proof}As before, we start by conditioning on the event $E_t$:
        \begin{align*}
            \E{\hat{r}_t(a) \given E_t} &= \E*{ \frac{r_t(a)\One{A^b_t=a}}{\hat{\pi}_t(a)} \given E_t } \\
            &= \E*{ \E[\Big]{\frac{r_t(a)}{\hat{\pi}_t(a)} \given A^b_t = a} \pi_b(a) \given E_t} \\
            &\geq \E*{ \frac{r_t(a)\pi_b(a)}{\pi_b(a)+\epsilon_t} \given E_t} \\
            &= \frac{r_t(a)}{1+\epsilon_t/\pi_b(a)} \\
            &\geq r_t(a)\left( 1- \frac{\epsilon_t}{\pi_b(a)}\right)
        \end{align*}
        Again, thanks to the Law of total expectation we have:
        \begin{align*}
            \E{\hat{r}_t(a)} &= \E{\hat{r}_t(a) \given E_t}\P{E_t} + \E{\hat{r}_t(a) \given \bar{E}_t}\P{\bar{E}_t}\\
                &\geq r_t(a) - r_t(a)\delta_t + \frac{\epsilon_t}{\pi_b(a)}(1-\delta_t) \\
                &\geq r_t(a) - \delta_t
        \end{align*}
    \end{proof}

\end{lemma}

\begin{lemma}
    $$
    \E{\ip{\pi^*}{\hat{r}^2_t}} \leq ?
    $$
\end{lemma}

